High-dimensional estimation with missing data: Statistical and computational limits

We consider computationally-efficient estimation of population parameters when observations are subject to missing data. In particular, we consider estimation under the realizable contamination model of missing data in which an $\epsilon$ fraction of the observations are subject to an arbitrary (and unknown) missing not at random (MNAR) mechanism. When the true data is Gaussian, we provide evidence towards statistical-computational gaps in several problems. For mean estimation in $\ell_2$ norm, we show that in order to obtain error at most $\rho$, for any constant contamination $\epsilon \in (0, 1)$, (roughly) $n \gtrsim d e^{1/\rho^2}$ samples are necessary and that there is a computationally-inefficient algorithm which achieves this error. On the other hand, we show that any computationally-efficient method within certain popular families of algorithms requires a much larger sample complexity of (roughly) $n \gtrsim d^{1/\rho^2}$ and that there exists a polynomial time algorithm based on sum-of-squares which (nearly) achieves this lower bound. For covariance estimation in relative operator norm, we show that a parallel development holds. Finally, we turn to linear regression with missing observations and show that such a gap does not persist. Indeed, in this setting we show that minimizing a simple, strongly convex empirical risk nearly achieves the information-theoretic lower bound in polynomial time.

==> macros.tex <==
\usepackage{enumerate}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{xifthen}
\usepackage{mathtools}
\usepackage{bbm}
\usepackage{thm-restate}
\usepackage{enumitem}
\usepackage{tikz}
\usepackage{subcaption}
\usepackage{turnstile} %
\usepackage{algpseudocode,algorithm,algorithmicx}  

\usepackage[
backend=biber,
natbib=true,
style=alphabetic,
maxbibnames=15,
maxalphanames=10,
minalphanames=6,
doi=false,
isbn=false,
url=false,
eprint=false,
backref=true,
]{biblatex}
\addbibresource{refs.bib}
\addbibresource{ref.bib}

\RequirePackage[colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref} %
\usepackage[capitalize]{cleveref}


\newcommand{\wt}{\widetilde}

\newcommand{\dimension}{d}

\newcommand{\R}{\mathbf{R}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\pE}{\widetilde{\mathbb{E}}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\eps}{\epsilon}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\diff}{\mathrm{d}}

\newcommand{\Var}{\mathrm{Var}}

\newcommand{\1}{\mathbf{1}}

\usepackage[draft,inline,nomargin,index]{fixme}
\fxsetup{theme=color,mode=multiuser}

\definecolor{darkgreen}{RGB}{0,100,0}

\newcommand{\shnote}[1]{ {\color{red}[SH: #1]}}

\newcommand{\kavnote}[1]{{\color{blue}[KV: #1]}}
\newcommand{\rknote}[1]{{\color{darkgreen}[RK: #1]}}
\newcommand{\apnote}[1]{{\color{purple}[AP: #1]}}



\makeatletter
\newcommand{\ostar}{\mathbin{\mathpalette\make@circled\star}}
\newcommand{\make@circled}[2]{%
  \ooalign{$\m@th#1\smallbigcirc{#1}$\cr\hidewidth$\m@th#1#2$\hidewidth\cr}%
}
\newcommand{\smallbigcirc}[1]{%
  \vcenter{\hbox{\scalebox{0.77778}{$\m@th#1\bigcirc$}}}%
}
\makeatother

\newcommand{\anote}[1]{\footnote{{\bf [Ankit: {#1}\bf ]}}}



\newcommand{\est}{\hat{\theta}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\let\vec\mathbf  %

\newcommand{\bA}{\vec{A}} \newcommand{\bB}{\vec{B}} \newcommand{\bC}{\vec{C}}
\newcommand{\bD}{\vec{D}} \newcommand{\bE}{\vec{E}} \newcommand{\bF}{\vec{F}}
\newcommand{\bG}{\vec{G}} \newcommand{\bH}{\vec{H}} \newcommand{\bI}{\vec{I}}
\newcommand{\bJ}{\vec{J}} \newcommand{\bK}{\vec{K}} \newcommand{\bL}{\vec{L}}
\newcommand{\bM}{\vec{M}} \newcommand{\bN}{\vec{N}} \newcommand{\bO}{\vec{O}}
\newcommand{\bP}{\vec{P}} \newcommand{\bQ}{\vec{Q}} \newcommand{\bR}{\vec{R}}
\newcommand{\bS}{\vec{S}} \newcommand{\bT}{\vec{T}} \newcommand{\bU}{\vec{U}}
\newcommand{\bV}{\vec{V}} \newcommand{\bW}{\vec{W}} \newcommand{\bX}{\vec{X}}
\newcommand{\bY}{\vec{Y}} \newcommand{\bZ}{\vec{Z}}

\newcommand{\ba}{\vec{a}} \newcommand{\bb}{\vec{b}} \newcommand{\bc}{\vec{c}}
\newcommand{\bd}{\vec{d}} \newcommand{\be}{\vec{e}} \newcommand{\bfm}{\vec{f}}
\newcommand{\bg}{\vec{g}} \newcommand{\bh}{\vec{h}} \newcommand{\bi}{\vec{i}}
\newcommand{\bj}{\vec{j}} \newcommand{\bk}{\vec{k}} \newcommand{\bl}{\vec{l}}
\newcommand{\bm}{\vec{m}} \newcommand{\bn}{\vec{n}} \newcommand{\bo}{\vec{o}}
\newcommand{\bp}{\vec{p}} \newcommand{\bq}{\vec{q}} \newcommand{\br}{\vec{r}}
\newcommand{\bs}{\vec{s}} \newcommand{\bt}{\vec{t}} \newcommand{\bu}{\vec{u}}
\newcommand{\bv}{\vec{v}} \newcommand{\bw}{\vec{w}} \newcommand{\bx}{\vec{x}}
\newcommand{\by}{\vec{y}} \newcommand{\bz}{\vec{z}}


\newcommand{\cA}{\mathcal{A}} \newcommand{\cB}{\mathcal{B}} \newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}} \newcommand{\cE}{\mathcal{E}} \newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}} \newcommand{\cH}{\mathcal{H}} \newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}} \newcommand{\cK}{\mathcal{K}} \newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}} \newcommand{\cN}{\mathcal{N}} \newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}} \newcommand{\cQ}{\mathcal{Q}} \newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}} \newcommand{\cT}{\mathcal{T}} \newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}} \newcommand{\cW}{\mathcal{W}} \newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}} \newcommand{\cZ}{\mathcal{Z}}
\newcommand{\Bin}{\mathsf{Bin}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\simiid}{\stackrel{\rm iid}{\sim}}

\newcommand{\mnar}{\mathsf{MNAR}}
\newcommand{\mcar}{\mathsf{MCAR}}
\newcommand{\law}{\mathsf{Law}}


\crefformat{equation}{(#2#1#3)}
\crefname{equation}{Equation}{Equations}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{claim}{Claim}{Claims}
\crefname{fact}{Fact}{Facts}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{remark}{Remark}{Remarks}
\crefname{definition}{Definition}{Definitions}
\crefname{question}{Question}{Questions}
\crefname{condition}{Condition}{Conditions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{figure}{Figure}{Figures}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{assumption1}[theorem]{Assumption}
\newtheorem{estimator}[theorem]{Estimator}
\newtheorem{condition}[theorem]{Condition}

\newtheorem{remark}[theorem]{Remark}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\reals}{\mathbb{R}}

\newcommand{\mc}{\mathcal}

\newcommand{\sos}[2]{\sststile{#2}{#1}}

\newcommand{\new}[1]{{\textcolor{blue}{ #1}}}


\newcommand{\iid}{\stackrel{\mathrm{i.i.d.}}{\sim}}
\newcommand{\supp}{\mathrm{supp}}

\newcommand{\KL}{\mathrm{KL}}

\newcommand{\STAT}{\mbox{STAT}}

\newcommand{\pobserved}{q}

\allowdisplaybreaks
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\Bern}{\mathsf{Bern}}
\newcommand{\SQtolerance}{\kappa}
\newcommand{\indep}{\perp \!\!\! \perp}

\newcommand{\Tstar}{T_{\mathsf{MCAR}}}%
\newcommand{\Tprime}{T_{\mathsf{MCAR}, \star}}%
\newcommand{\Tdprime}{T_{\mathsf{MNAR}}}%

